Proving Termination of Probabilistic Programs Using Patterns

Proving programs terminating is a fundamental computer science challenge. Recent research has produced powerful tools that can check a wide range of programs for termination. The analog for probabilistic programs, namely termination with probability one ("almost-sure termination"), is an equally important property for randomized algorithms and probabilistic protocols. We suggest a novel algorithm for proving almost-sure termination of probabilistic programs. Our algorithm exploits the power of state-of-the-art model checkers and termination provers for nonprobabilistic programs: it calls such tools within a refinement loop and thereby iteratively constructs a "terminating pattern", which is a set of terminating runs with probability one. We report on various case studies illustrating the effectiveness of our algorithm. As a further application, our algorithm can improve lower bounds on reachability probabilities.

==> app-computing.tex <==
\subsection{Proofs of Section~\ref{sec:computing}}
 \label{app:computing}

\begin{qproposition}{\ref{prop:finitealgo}}
 \stmtpropfinitealgo
\end{qproposition}

\begin{proof}
%We claim that if $P$ is a.s.-terminating, then the pattern checker eventually shows termination,
% i.e., the pattern $\Seq(s_j, s_j, \ldots)$ is terminating for some $j \in \mathbb{N}$.
Recall from the proof of Theorem~\ref{th:coinPattern}~(3) that there is a fixed word $z \in C^*$
 which leads from an arbitrary node in $\Runs(\mathcal{M}_P)$ to termination.
In particular, $z$ is never an infix of $u_i^\omega$ for any~$i$.
It follows that $s_0 z$ is never an infix of $u_i^\omega$ for any~$i$.
Assume for a contradiction that our algorithm does not succeed in proving termination.
Since the $s_i$ are all pairwise different, our algorithm eventually chooses $s_j := s_0 z$ for some $j \in \mathbb{N}$.
By the definition of~$z$ the pattern $C^* z C^* z \ldots$ is terminating,
 hence so is $C^* s_j C^* s_j \ldots$
It follows that the pattern checker shows $P_{j+1}$ terminating, which is a contradiction.
\qed
\end{proof}

\begin{qproposition}{\ref{prop:shortword}}
 \stmtpropshortword
\end{qproposition}
\begin{proof}
If a word~$w$ is not an infix of any of the words $u_1^\omega$, \ldots, $u_j^\omega$,
 then neither is $s_0 w$.
Hence it suffices to construct such a word~$w$ with $|w| \le 1 + \log_2 K$, where $K := |u_1| + \cdots + |u_j|$.
Let $p_1, \ldots, p_{K}$ be an enumeration of all suffixes of the words $u_1^\omega, \ldots, u_j^\omega$.
For any word~$w$, denote by $S(w) \subseteq \{p_1, \ldots, p_K\}$ the set of words $p \in \{p_1, \ldots, p_K\}$
 such that $w$ is a prefix of~$p$.
It suffices to construct~$w$ such that $|w| \le 1 + \log_2 K$ and $S(w) = \emptyset$.
We construct~$w$ iteratively.
Let $w_0 := \epsilon$.
In each iteration~$i$, choose $w_{i+1} := w_{i} c$ with $c \in \{0, 1\}$
 so that $|S(w_{i} c)|$ is minimized.
Observe that $|S(w_{i+1})| \le |S(w_{i})| / 2$, as all words in~$S(w_{i})$ start with either $w_{i} 0$ or~$w_{i} 1$.
It follows that $S\left(w_{1 + \lfloor \log_2 K \rfloor}\right) = \emptyset$.
\qed
\end{proof}


==> app-nondet.tex <==


\section{Patterns for Nondeterministic Programs}
\label{app:response}

% \begin{figure}[tbp]
% \centering
%  \tikzset{
%    dim/.style={
%            rounded corners,
%            minimum height=2em,
%            inner sep=2pt,
%            text centered,
%            },
%     state/.style={
%            rectangle,
%            rounded corners,
%            draw=black, very thick,
%            minimum height=2em,
%            inner sep=2pt,
%            text centered,
%            },
%    act/.style={
%            circle,
%            draw=black, very thick,
%            minimum height=2em,
%            inner sep=2pt,
%            text centered,
%            },
%   fail/.style={circle, double, draw=black, inner sep=2pt, minimum height=2em, very thick},
%   nothing/.style={
%            rectangle,
%            rounded corners,
%            minimum height=2em,
%            inner sep=0pt,
%            text centered,
%            }
%   }
% \scalebox{0.6}{
% \centering
% \begin{tikzpicture}[->,>=stealth',scale=1,font=\Large]
%
%  \node[dim, anchor=center] (S1)
%  {$ $};
%
%  \node[act] (L0) [right =of S1]
%  {$\bot$};
%
%  \node[act] (L1) [right =3.5cm of L0]
%  {$l_1$};
%
%  \node[act] (L2) [right =3.5cm of L1]
%  {$l_2$};
%
%  \node[act] (TOP) [right =3cm of L2]
%  {$\top$};
%
%  % draw the paths and and print some Text below/above the graph
%  \path[very thick]
%        (S1) edge[above] node [above] {$ $} (L0)
%        (L0) edge[above] node [below] {$x := \nondet()$} (L1)
%        (L1) edge[above] node [below] {$y := \coin(p)$} (L2)
%        (L2) edge node [below] {$x \not= y?$} (TOP)
%         (L2) edge[bend right=25] node [above] {$x = y?$} (L0)
%        (TOP) edge[loop below] node [right] {} (TOP);
% \end{tikzpicture}
% }
% \caption{A.s.-terminating program without terminating coin pattern.}\label{fig:coinPatternCounterExample}
% \end{figure}
%
For general a.s.-terminating probabilistic programs, there might not exist a terminating pattern, even if
the program is finite, recall Figure~\ref{fig:coinPatternCounterExample}.

We therefore propose another pattern class that also takes nondeterministic decisions into account.
We fix an arbitrary probabilistic program~$P = (\mathcal{L}, I, \mathord{\hookrightarrow}, \lab, \bot, \top)$,
and its associated MDP $\mathcal{M}_P =  (Q_A, Q_P, \text{Init}, \mathord{\rightarrow}, \text{Lab}_A, \text{Lab}_P)$.
We assume that $P$ is in a special \emph{normal form}: Every nondeterministic location has a probabilistic location as its successor, every
probabilistic location has a nondeterministic location as its successor. It is easy to transform a program in normal form by adding
redundant probabilistic and nondeterministic locations such that the transformed program terminates if{}f the original one does.
For example, the program in Fig.~\ref{fig:coinPatternCounterExample} is in normal form.
%Note that for every run $r \in \mathcal{M}_P$, it holds that $r|_G \in (A C)^\infty$ if $P$ is in normal form.
If $P$ is in normal form, then every run $r \in \mathcal{M}_P$ satisfies $r|_G \in (A C)^\infty$.

We write $A := \{a_0, a_1\}$ and $G := \{a_0, a_1\} \cup C$.
A set $W \subseteq (A C)^*$ is called a \emph{response} of length~$n \geq 0$ if
(i) every $w \in W$  has length $2n$,
(ii) for $w_1, w_2 \in W$ with $w_1 \not= w_2$, $w_1|_A \not= w_2|_A$ holds, and (iii) $W$ contains exactly $2^n$ elements.
We denote by $\Resp(n)$ the set of responses of length~$n$, and set $\Resp := \bigcup_{n \in \mathbb{N}}{\Resp(n)}$.
Intuitively, a response $R$ of length~$n$ contains for every sequence of nondeterministic actions of length $n$ a sequence of
coin toss outcomes of length $n$ (interleaved in one word of $R$). For example,
$\{a_0c_1, a_1c_0\}$ is a response of length one, $\{a_0c_0a_0c_1, a_0c_0a_1c_1, a_1c_0a_0c_1, a_1c_0a_1c_1\}$ is a response
of length two.

A \emph{response pattern} is a subset of $(A C)^\omega$ of the form $(A C)^* R_1 (A C)^* R_2 (A C)^* \ldots$, where $R_1, R_2, \ldots$ are responses.
We say $R_1, R_2, \ldots$ induces the response pattern.

As in the deterministic case,
fixing an enumeration $R_1, R_2, \ldots$ of all responses, we call the pattern $(A C)^* R_1 (A C)^*R_2(A C)^*$ a \emph{universal response pattern}.
For a response pattern~$\Phi$, a run $r \in \Runs(\mathcal{M}_P)$ is $\Phi$-conforming if there is $v \in \Phi$ such that $\bar{r}|_G$ is a prefix of $v$.
We call a response pattern $\Phi$ \emph{terminating} if all $\Phi$-conforming runs terminate.

Analogously to the deterministic case,
we show the following theorem in Appendix~\ref{app:responseProofs}:
\newcommand{\stmtthmresponsePattern}{
Let $P$ be a probabilistic program in normal form.
\begin{itemize}
\item[(1)]
 Let $\Phi$ be a response pattern.
 The set of $\Phi$-conforming runs has probability~$1$ for every strategy $S$ for $\mathcal{M}_P$.
 In particular, if $P$ has a terminating pattern, then $P$ is a.s.-terminating.
\item[(2)]
 If $P$ is a.s.-terminating and weakly finite, then the universal pattern is terminating for~$P$.
\item[(3)]
 If $P$ is a.s.-terminating and finite with $n < \infty$ reachable nodes in~$\mathcal{M}_P$,
  then there exists a response $R$ of length in $\mathcal{O}(n^2)$ such that $(A C)^* R (A C)^\omega$ is terminating for~$P$.
\end{itemize}
}
\begin{theorem} \label{th:responsePattern}
 \stmtthmresponsePattern
\end{theorem}
%
% \begin{example}
%  For the program in Fig.~\ref{fig:coinPatternCounterExample}, a terminating response pattern is $\Phi = (A C)^* \{a_0c_1, a_1c_0\} (A C)^\omega$.
%   Every $\Phi$-conforming run has the form
% \begin{equation*}
%  \tup{\top, \sigma_0} \rightarrow \ldots \rightarrow q \xrightarrow {a_{i} } q' \xrightarrow {c_{1-i}} q'' \rightarrow \top  \rightarrow \ldots
%  \qquad \text{for an $i \in \{0,1\}$.}
% \end{equation*}
% \end{example}




==> app-patterns.tex <==
% todo:
% Definiere \circ, follow allgemein
% Zusammenfassen
% Verweis auf Beweise im Haupttext
% Beweis für NONDET weakly finite
\section{Proofs}

\section{Preliminaries}
Let~$P = (\mathcal{L}, I, {\hookrightarrow}, \lab, \bot, \top)$, and let $\mathcal{M}_P$ be its corresponding
MDP with $\mathcal{M}_P = (Q_A, Q_D, \text{Init}, \rightarrow, \text{Lab}_A, \text{Lab}_P)$.

The probability $\Pr[q_1 \xrightarrow l q_2]$ of a transition $q_1 \xrightarrow {l,p} q_2$ is equal to~$p$.
We define a probability measure on the set of runs of a Markov chain $\mathcal{M}$ in the usual way (see e.g.~\cite{principlesMC}).
The \emph{cylinder set} $\cyl{\pi}$ of a path~$\pi$ is the set of runs having $\pi$ as prefix.
The probability of $\cyl{\pi}$ for a path $\pi$ starting at $q$, denoted by $\Pr_{q}[\cyl{\pi}]$, is $1$ if $\pi = q$,
and otherwise the product of the probabilities of the transitions of $\pi$.
There is a unique extension of $\Pr_{q}$ to a probability measure
over the smallest $\sigma$-algebra $\mathfrak{S}^{\mathcal{M}}$
containing all cylinder sets starting at $q$. We denote it by $\Pr_{q}$. We say a set of runs is $\emph{measurable}$ if it
is contained in $\mathfrak{S}^{\mathcal{M}}$.

For general MDPs, we can only define a probability measure after resolving the nondeterminism.
A \emph{strategy} for an MDP~$\mathcal{M}$ is a function $S$ that maps the empty path
$\epsilon$ to an initial node $q_0$, and every path
$q_0 \xrightarrow {l_0} q_1 \cdots q_{n-1} \xrightarrow {l_{n-1}} q_n \in \Paths(\mathcal{M})$
 ending at an action node to a probability distribution over the outgoing labels of $q$, i.e.,
over the labels $l$ such that $q_n \xrightarrow l q$ for some node $q$. Given a strategy
$S$, we define the Markov chain $\mathcal{M}[S]$
as usual (see \cite{principlesMC} for a formal definition): the nodes of $\mathcal{M}[S]$
are the paths of $\mathcal{M}$ whose cylinders have nonzero probability, the transitions
are defined to match the definition of the nodes, and the transition probabilities are
assigned according to $S$. For every node $q$ of $\mathcal{M}$ we define a probability measure $\Pr_q^S$ over $\mathfrak{S}^{\mathcal{M}}$,
that assigns to a cylinder $\cyl{\pi}$ the probability
of $\cyl{\pi'}$ in the Markov chain $\mathcal{M}[S]$,
 where $\pi'$ is the unique path of $\mathcal{M}[S]$ starting at the node $q$ (notice that $q$ is also a path, and so a node of~$\mathcal{M}[S]$)
 and ending at the node $\pi$. We write $\Pr^S[\cdot]$ for $\Pr^S_{q_0}[\cdot]$.



\section{Proofs of Section~\ref{sec:patterns}} \label{app-patterns}

\subsection{Proof of Theorem~\ref{th:coinPattern}}



In this section we complete the proof of
\begin{qtheorem}{\ref{th:coinPattern}} \mbox{}
Let $P$ be a probabilistic program that is deterministic.
 \stmtthmcoinPattern
\end{qtheorem}

\begin{proof}
It remains to prove parts (1) and (3).
Let~$P = (\mathcal{L}, I, {\hookrightarrow}, \lab, \bot, \top)$,
and its corresponding MDP be $\mathcal{M}_P =  (Q_A, Q_P, \text{Init}, \mathord{\rightarrow}, \text{Lab}_A, \text{Lab}_P)$.

Let $\Phi = C^*w_1C^*w_2C^* \ldots$; the set of runs conforming to $\Phi$ are denoted by $\Runs(\Phi)$.


% At first we require an
% \paragraph{Observation.}

% \qed


\subsubsection{Proof of Part (1):} $ $ \\

Let \emph{$I_C \in \mathfrak{S}^{\mathcal{M}_P}$} be the set of runs $r$ with $\bar{r}|_C \in C^\omega$.
For  $w_1, w_2, \ldots w_i$, $i \geq 1$, we define the set
\emph{$S(w_1, w_2, \ldots, w_i)$} by
\begin{equation*}
 S(w_1, w_2, \ldots, w_i) := \{ r \in \Runs(\mathcal{M}_P) \mid \bar{r}|_M \in C^* w_1 C^* w_2 C^* \ldots C^* w_i C^\omega \}.
\end{equation*}
$S(w_1, w_2, \ldots, w_i)$ is measurable:
Let $\text{NC}(i) \in \mathfrak{S}^{\mathcal{M}_P}$ be the set of all runs $r$ with the $i$-th label of $r$ not in $C$, and
$F(i, c)\in \mathfrak{S}^{\mathcal{M}_P}$ the set of runs that have $c$ as $i$-th label. Set
\begin{equation*}
 G(b^-,b^+, c_1 \ldots c_k) =  \bigcup_{b^- \leq a_1 < \ldots < a_k < b^+} \Big(
 \bigcap_{\substack{l > a_1 \\ \wedge l \not \in \{a_1, \ldots, a_k\}}}{\text{NC}(l)} \cap \bigcap_{1 \leq j \leq k} {F(a_j, c_j)} \Big) \in \mathfrak{S}^{\mathcal{M}_P}
\end{equation*}
for $\{b^-,b^+,k\} \subseteq \mathbb{N}$ and $c_1 \ldots c_k \in C^k$. $S(w_1, w_2, \ldots, w_n)$ can be written as
\begin{equation*}
I_C \cap  \bigcup_{0 \leq b^-_1 < b^+_1 < b^-_2 < \ldots < b^-_{n} < b^+_n} {G(b^-_1, b^+_1, w_1) \cap \ldots \cap G(b^-_{n}, b^+_n, w_n)} \in \mathfrak{S}^{\mathcal{M}_P}.
\end{equation*}
Since
\begin{equation*}
 \Runs(\Phi) = \Big( \Runs(\mathcal{M}_P) \setminus I_C\Big) \cup \bigcap_{i\geq 0}{S(w_1, w_2, \ldots, w_i)}  \in \mathfrak{S}^{\mathcal{M}_P}
\end{equation*}
we conclude that $\Runs(\Phi)$ is also measurable.

Next we show that $Pr[\Runs(\Phi)] = 1$.

For every prefix $w_1, w_2, w_3, \ldots, w_i$ of $(w_i)_{i \in \mathbb{N}}$,
$\Pr[S(w_1, \ldots, w_i)] =  \Pr[I_C]$ holds, i.e.,
the set of runs that visit probabilistic nodes infinitely often, but
are \emph{not} $C^*w_1C^*w_2C^*\ldots C^*w_iC^\omega$-conforming, have probability zero.

For proving this we write $w = w_1w_2\ldots w_i$. Let $n = \abs{w}$.
$S(w) \subseteq S(w_1, w_2, \ldots, w_i)$ holds for all $i$.
It suffices to show that $\Pr[S(w)] = \Pr[I_C]$, since this implies with $I_C \supseteq S(w_1, \ldots, w_i)$ that $\Pr[I_C] = \Pr[S(w_1, w_2, \ldots, w_i)]$.

Let $V(j)$ be the set of runs that visit a probabilistic node at least $j$ times,
and let
\begin{equation*}
B(j) =  V(j\cdot n) \cap (\Runs(\mathcal{M}_P) \setminus S(w))
\end{equation*}
be the set of runs $r$ that visit a probabilistic node at least $j\cdot n$ times, and $w$ is no substring of $\bar{r}|_C$.


%%
Since there are only finitely many probabilistic locations in $P$, there exists a minimal probability $p_{min} > 0$ such that for every
transition $q \xrightarrow {c,p'} q'$, $c \in \{0, 1\}$, $p' \geq p$ holds.
For $x \in C^*$ we write $\text{NV}(x)$(``not visited'') for the set of runs $r$ such that $\bar{r}|_C$ does not contain $x$ as a substring.
Now
\begin{align*}
 & Pr[B(1)] & \\
  &= Pr[\text{NV}(w) \mid V(n)] \cdot Pr[V(n)]& \\
%  &\leq \sum_{w \in R} Pr^S[\text{NV}(w) \mid SC(w|_A)  \cap V(n)]  \cdot Pr^S[SC(w|_A) \cap V(n)]& \\
  &\leq (1-p_{\min}^n) \cdot Pr[V(j)] & \\
  &\leq (1-p_{\min}^n),
\end{align*}
%%
i.e.,
after visiting probabilistic nodes at least $n$ times, the probability $p$ of \emph{not} seeing the sequence $w$ is at most $(1-p_{min}^n) < 1$.
With a simple inductive argument we obtain $Pr[B(j)] \le (1-p_{\min}^n)^j$.
It holds that $B(j) \supseteq B(j+1)$ for all $j$. Then
\begin{equation}
\label{eq:pr-b-is-zero}
Pr[\bigcap_{j \geq 1}{B(j)}] =  \lim_{j \rightarrow \infty}{Pr[B(j)]} \leq \lim_{j \rightarrow \infty}{(1-p_{min}^n)^j} = 0.
\end{equation}
We can write $S(w) = I_C \setminus \bigcap_{j \geq 0}{B(j)}$.
Hence
\begin{align*}
 Pr[S(w_1w_2 \ldots w_i)]] &= Pr[I_C \setminus \bigcap_{j \geq 1}{B(j)}] &  \text{(Def. of $B(\cdot)$)}\\
 &= Pr[I_C] - Pr[\bigcap_{j \geq 1}{B(j) \cap I_C}] &\\
 &= Pr[I_C] & \text{(Eq.~\ref{eq:pr-b-is-zero}).}
\end{align*}


Now $Pr[I_C \setminus S(w_1, \ldots, w_i)] = Pr[I_C] - Pr[S(w_1, \ldots, w_i)] = 0$.
We can write
\begin{equation*}
 I_C \setminus \bigcap_{i\geq1}{S(w_1, \ldots, w_i)} = I_C \cap \bigcup_{i \geq 1}{I_C \setminus S(w_1, \ldots, w_i)}.
\end{equation*}
For every $i \geq 1$, $I_C \setminus S(w_1, \ldots, w_i)$ is a null set, thus the countable union
$\bigcup_{i \geq 1}{I_C \setminus S(w_1, \ldots, w_i)}$ is also a null set (*).

We conclude:
\begin{align*}
  & Pr[\Runs(\Phi)] & \\
  &= Pr[\Runs(\mathcal{M}_P) \setminus I_C] + Pr[\bigcap_{i\geq 0}{S(w_1, \ldots, w_i)} ] & \\
  &= Pr[\Runs(\mathcal{M}_P) \setminus I_C] + Pr[I_C] & \text{ (*)}\\
  &= 1.
\end{align*}

\subsubsection{Proof of Part (3):} $ $ \\

We say that $q \in Q$ \emph{ends up in} $q' \in Q$ \emph{following} $w = c_1 c_2 \ldots c_m \in C^*$ if
\begin{equation*}
 q \xrightarrow {\tau^* c_1 \tau^* c_2 \tau^* \ldots \tau^* c_m  \tau^*} q',
\end{equation*}
with $q'$ probabilistic or $\top$. Note that $q'$ is unique if it exists.

For every reachable node $q$ and every sequence $w \in C^*$ holds that either:
(i) $q$ ends up in a node following $w$, or (ii) $q$ ends up in $\top$
following a prefix of $w$. Otherwise there exists a node $q'$ from which no probabilistic location or $\top$ is reachable any more, which contradicts
that $P$ is a.s.-terminating.

For every node $q \in Q$, there exists a $w_q = c_1c_2\ldots c_m \in C^*$ such that
$q$ ends up in $\top$ following $w_q$, again due to the a.s.-termination property of $P$. We can choose $w_q$ such
that $\abs{w_q} < n$ by removing cycles.

We construct a sequence $w^{(0)},w^{(1)},\ldots, w^{(m)} $ using the following algorithm.
Set $w^{(0)} := \epsilon$ and $i := 1$.
\begin{enumerate}
\item Pick a $q'_i \in Q$ that does end up in a node $q_i \not= \top$ following $w^{(i-1)}$. If no such $q_i$ exists set $w := w^{(i-1)}$ and terminate.
\item Set $w^{(i)} := w^{(i-1)} w_{q_i}$. Set $i := i+1$ and go to 1).
\end{enumerate}

The node set $Q^{(i)}$ in which a node of $Q$ might end up after following $w^{(i)}$ contains at most $n-i$
nodes.
This is certainly true for $i = 0$.
In the $i$-th iteration the chosen $q'_i$ ends up in $q_i \in Q^{(i-1)}$
after following $w^{(i-1)}$. After following $w_{q_i}$, $q_i$ ends up in $\top$. Thus $q_i$ ends up in $\top$ after $w^{(i)}$. This implies that
$\abs{Q^{(i)}} < \abs{Q^{(i-1)}}$, since every node can end up in at most one node after following a nonempty coin sequence, and note that
every $Q^{(i)}$ contains $\top$.

After at most $n-1$ iterations, $\abs{Q^{(i)}} \leq 1$, and the algorithm terminates. Hence $\abs{w} \leq (n-1)\cdot \max_{q\in Q}{\abs{w_q}} \leq (n-1)^2$.
Every node of $Q$ ends up in $\top$ after following a prefix of $w^{(i)}$. If it ended up in another node $\hat{q}$, the algorithm would have
performed another iteration, making $w$ longer, if there were no node $q'$such that $q$ ends up in $q'$, a prefix of $w$ must have led it to $\top$ before.

We can conclude that every run $r$ for which $\bar{r}|_C$ is a prefix of a word $C^* w C^\omega$ is terminating, and thus $C^* w C^\omega$ is a terminating pattern.
$ $
\qed
\end{proof}



% Fully nondeterministic Section
%
%
%


\section{Proofs of Section~\ref{sec:responsePatterns}}


In this section we prove

%\begin{qtheorem}{\ref{th:responsePattern}} \mbox{}
% \stmtthmresponsePattern
%\end{qtheorem}

\begin{proof}
Let~$P = (\mathcal{L}, I, {\hookrightarrow}, \lab, \bot, \top)$.

The MDP corresponding to~$P$ is denoted by $\mathcal{M}_P = (Q_A, Q_D, \text{Init}, \rightarrow, \text{Lab}_A, \text{Lab}_P)$.
We write $Pr[\cdot]$ for $Pr_{q_I}[\cdot]$.

Let $\Phi = (A C)^* R_1 (A C)^* R_2 \ldots$, with $R_i$ a response for all $i \geq 1$.
Again we call the set of $\Phi$-corresponding runs $\Runs(\Phi)$.

For responses $R_1, R_2$ of length $n_1$ and $n_2$, respectively, and a word $w \in (A C)^+$, we set
$w \circ R_1 := \{ w r \mid r \in R_1 \} \text{ and } R_1 \circ R_2 := \{ r R_2 \mid r \in R_1\}$.
$R_1 \circ R_2$ is a response of length $n_1+n_2$.

Let $\Phi = C^*w_1C^*w_2C^* \ldots$; the set of runs conforming to $\Phi$ are again denoted by $\Runs(\Phi)$.


\subsection{Proof of Part (1):}

Let \emph{$I_G \in \mathfrak{S}^{\mathcal{M}_P}$} be the set of runs $r$ with $\bar{r}|_G \in G^\omega$.
For  $R_1, R_2, \ldots R_i$, $i \geq 1$, we define the set
\emph{$S(R_1, R_2, \ldots, R_i)$} by
\begin{equation*}
 S(R_1, R_2, \ldots, R_i) := \{ r \in \Runs(\mathcal{M}_P) \mid \bar{r}|_M \in G^* R_1 C^* R_2 G^* \ldots G^* R_i G^\omega \}.
\end{equation*}
$S(R_1, R_2, \ldots, R_i)$ is measurable:
The set of runs $r$ such that $\bar{r}|_M \in G^* w_1 C^* w_2 G^* \ldots G^* w_i G^\omega$ for $(w_1, \ldots, w_i) \in R_1 \times \ldots \times R_i$ is measurable,
which can be proved by an easy variation of the first part of the proof in Theorem~\ref{th:coinPattern}.
$S(R_1, R_2, \ldots, R_i)$ is the finite union of all these run sets and thus measurable.
Again, since
\begin{equation*}
 \Runs(\Phi) = \Big( \Runs(\mathcal{M}_P) \setminus I_C\Big) \cup \bigcap_{i\geq 0}{S(R_1, R_2, \ldots, R_i)}  \in \mathfrak{S}^{\mathcal{M}_P}
\end{equation*}
we conclude that $\Runs(\Phi)$ is  measurable.

Let now $S$ be a strategy for $\mathcal{M}_P$.
We show that $Pr^S[\Runs(\Phi)] = 1$, again reusing ideas from the proof of Theoren~\ref{th:coinPattern}.


For every prefix $R_1, R_2, R_3, \ldots, R_i$ of $(R_i)_{i \in \mathbb{N}}$,
$\Pr[S(R_1, \ldots, R_i)] =  \Pr[I_C]$ holds, i.e.,
the set of runs that visit probabilistic nodes infinitely often, but
are \emph{not} $C^*w_1C^*w_2C^*\ldots C^*w_iC^\omega$-conforming, have probability zero.

For proving this we write $R = R_1R_2\ldots R_i$. Let $n$ be the resulting length of $R$.
$S(R) \subseteq S(R_1, R_2, \ldots, R_i)$ holds for all $i$.
Again it suffices to show that $\Pr[S(R)] = \Pr[I_G]$. %, since this implies with $I_C \supseteq S(w_1, \ldots, w_i)$ that $\Pr[I_C] = \Pr[S(w_1, w_2, \ldots, w_i)]$.

We reuse the definition of the sets
$V(j)$, containing the set of runs that visit a probabilistic node at least $j$ times,
and set
\begin{equation*}
B(j) =  V(j\cdot n) \cap (\Runs(\mathcal{M}_P) \setminus S(R))
\end{equation*}
the set of runs $r$ that visit a probabilistic node at least $j\cdot n$ times, and \emph{no} $w \in R$ is a substring of $\bar{r}|_G$.
Recall that there exists a minimal probability $p_{min} > 0$ such that for every
transition $q \xrightarrow {c,p'} q'$, $c \in \{0, 1\}$, $p' \geq p$ holds.
For $x \in A^*$ we write $SC(x)$ (``strategy choice'') for the set of runs $r$ such that $\bar{r}|_A$ starts with $x$,
and $\text{NV}(x)$(``not visited'') for the set of runs $r$ such that $\bar{r}|_A$ does not contain $x$ as a substring.
Note that for $w \not= w'$ with $w,w'$ having the same
length,
\begin{equation}
 \label{eq:SCdisjunct}
  SC(w) \cap SC(w') = \emptyset.
\end{equation}
Now
\begin{align*}
 & Pr^S[B(1)] & \\
  &= \sum_{w \in R} Pr^S[\text{NV}(w) \mid \text{SC}(w|_A) \cap V(n)] \cdot Pr^S[\text{SC}(w|_A) \cap V(n)]& \\
%  &\leq \sum_{w \in R} Pr^S[\text{NV}(w) \mid SC(w|_A)  \cap V(n)]  \cdot Pr^S[SC(w|_A) \cap V(n)]& \\
  &\leq \sum_{w \in R} (1-p_{\min}^n) \cdot Pr^S[SC(w|_A) \cap V(j)] & \text{Eq. \ref{eq:SCdisjunct}}\\
  &\leq (1-p_{\min}^n).
\end{align*}
Again we can see that after visiting probabilistic nodes at least $n$ times, the probability of \emph{not} seeing at least \emph{one} of the $w \in R$ is at most $(1-p_{min}^n) < 1$.
In $B(j)$, we repeat this
experiment at least $j$ times; by a simple inductive argument we get again $Pr^S[B(j)] \le (1-p_{min}^n)^j$.
Now we proceed exactly as in the proof of Theorem~\ref{th:coinPattern}, substituting $Pr[\cdot]$ by $Pr^S[\cdot]$, $I_C$ by $I_G$, and $S(w_1, \ldots w_i)$ by $S(R_1, \ldots, R_i)$,
and obtain $Pr^S[I_G] = Pr^S[\bigcap_{i \geq 0}{S(R_1, \ldots, R_i)}]$. We conclude
\begin{align*}
  & Pr^S[\Runs(\Phi)] & \\
  &= Pr^S[\Runs(\mathcal{M}_P) \setminus I_G] + Pr^S[\bigcap_{i\geq 0}{S(R_1, \ldots, R_i)} ] & \\
  &= Pr^S[\Runs(\mathcal{M}_P) \setminus I_G] + Pr^S[I_G] & \\
  &= 1.
\end{align*}


\subsection{Proof of Part (2):}

The proof is analogously to the one of Theorem~\ref{th:coinPattern}, part (2):
Let $\sigma_1, \sigma_2, \ldots$ be a (countable or infinite) enumeration of the nodes in $I$.
With Part~(3) we obtain for each $i \geq 1$ a response $R_i$ such that $(AC)^* R_i (AC)^\omega$ is a terminating pattern for $P$,
if the only starting node considered is $\sigma_i$.
By its definition, the universal pattern is a subset of $(AC)^* R_i (AC)^\omega$ for every $i \ge 1$, so it is also terminating.

\subsection{Proof of Part (3):}


We reintroduce several notations from the proof of Theorem~\ref{th:coinPattern} and generalize them to accomodate nondeterminism.
We say now that $q \in Q$ \emph{ends up in} $q' \in Q$ \emph{following} $w = x_1 x_2 \ldots x_m \in G^*$ if
\begin{equation*}
 q \xrightarrow {\tau^* x_1 \tau^* x_2 \tau^* \ldots \tau^* x_m  \tau^*} q',
\end{equation*}
with $q'$ probabilistic, nondeterministic, or $\top$. Again, $q'$ is unique if it exists.

For every reachable node $q$ and every sequence $w \in G^*$ holds that either:
(i) $q$ ends up in a node following $w$, or (ii) $q$ ends up in $\top$
following a prefix of $w$. Otherwise there exists a node $q'$ from which no probabilistic or nondeterministic location or $\top$ is reachable any more, which contradicts
that $P$ is a.s.-terminating (note that there always exists a strategy that is able to cause $q_0$ ending up in $q'$ with nonzero probability, using
the nondeterministic choices given in $w$).


We show that for every node $q \in Q_A$ and every sequence $s_1 \ldots s_n \in A^n$
there exists a $c_1 c_2 \ldots c_n$ such that
$q$ ends up in $\top$ following $s_1 c_1 \ldots s_n c_n$ or a prefix of it.
Recall for the following that $P$ is in normal form, hence for every run $r$ it holds that $\bar{r}|_G \in (A C)^\omega \cup (A C)^*$.

Assume for the sake of contradicition
that there exists $q \in Q_A$ and a sequence  $s_1 \ldots s_n \in A^n$ such that no
$c_1 \ldots c_n$ exists with the property described above.
%%
We will construct a strategy $S$ such that (i) reaching $q$ has probability $> 0$,
(ii) every run reaching $q$ will never reach $\top$.
The probability of reaching $\top$ is then smaller than 1, contradicting the assumption that $P$ is a.s.-terminating.
Recall that nodes of $\mathcal{M}_P[S]$ are paths in $\mathcal{M}_P$.
Since $q$ is reachable in $\mathcal{M}_P$, there exists a cycle-free path $\pi$ from the initial node $q_0$ to $q$.
For all proper path prefixes of $\pi$ ending in a nondeterministic node, $S$ selects the choices contained in $\pi$ with probability 1, and
thus we reach $q$ with probability $> 0$.

For (ii), let $\pi$ be a path having the form $\pi = \pi' \rightarrow q_1 \xrightarrow {l_1} q_2 \xrightarrow {l_2} \ldots \xrightarrow {l_m} q_m$, with $m \geq 1$ and $q_1 = q$, such that $\pi'$ does not contain $q$.
We define $S(\pi)$ as follows:
Let $\pi_{r}$ be the path obtained from $q_1 \xrightarrow {l_1} q_2 \xrightarrow {l_2} \ldots \xrightarrow {l_m} q_m$ by removing all possible cycles.
$\pi_r$ then contains $k < n$ nondeterministic
nodes (there are only $n$ nodes in total). Set $S(\pi)(s_k) = 1$.
There is no path starting from a reachable state $\pi' \rightarrow q$ in $\mathcal{M}_P[S]$ that reaches $\top$, contradicting the assumption that $P$ is a.s.-terminating.
%%

We select a $c_1 \ldots c_n$ with the property described above for each $q \in Q_A$ and $s_1 \ldots s_n$, and set  $tr(q, s_1\ldots s_n) := s_1 c_1 \ldots s_n c_n$  and define
\begin{equation*}
 R(q) := \{ t(q, w) \mid w \in A^n \}.
\end{equation*}
Note that every $R(q)$ is a response. For every $w \in R(q)$, $q$ ends up in $\top$ following $w$ or a prefix of $w$. We say that a response with this property
\emph{leads} $q$ to $\top$.
%Every state $q' \in Q_P$ has a unique predecessor $q' \in Q_A$; hence $q'$ ends up in $\top$ after following  $w$a word in $R(q)$

We construct now a sequence $R^{(0)},R^{(1)},\ldots, R^{(m)} $ using the following algorithm.
Set $R^{(0)} := \emptyset$ and $i := 1$.
\begin{enumerate}
\item Pick a $q'_i \in Q_A$ that does end up in a node $q_i \not= \top$ following a $w \in R^{(i-1)}$. If no such $q_i$ exists set $R := R^{(i-1)}$ and terminate.
\item Set $R^{(i)} := (R^{(i-1)} \setminus {w}) \cup {w \circ R(q_i)}$. Set $i := i+1$ and go to 1).
\end{enumerate}

After performing the algorithm, we replace every
$w \in R$ such that $\abs{w} = k\cdot n < n^2$ by $w \circ R'$, with $R'$ an arbitrary
response of length $(n-k) \cdot n$, to obtain equal length of all words in $R$.


The node set $Q^{(i)}$ in which a node of $Q_A$ might end up after following a $w \in R^{(i)}$ contains at most $n-i$
nodes. Note that $Q^{(i)} \subseteq Q_A \cup \{\top\}$, since $P$ is in normal form.
This is certainly true for $i = 0$.
In the $i$-th iteration $q'_i$ ends up in $q'_i \in Q^{(i-1)}$
after following a $w \in R^{(i-1)}$. $R(q_i)$ leads $q_i$ to $\top$.
Thus $q'_i$ is lead to $\top$ by $R^{(i)}$.

This implies that
$\abs{Q^{(i)}} < \abs{Q^{(i-1)}}$: $q'_i \not= \top$ was contained in $\abs{Q^{(i)}}$, but is led to $\top$ by $R^{(i)}$, and therefore is not contained in
$Q^{(i)}$, everything else stays the same. Recall again that $\top$ is in every set $Q^{(j)}$ for $j \geq 0$.

Therefore, after at most $n-1$ iterations the algorithm terminates.
The length of the resulting $R$ is $n^2$, since every response $R(q)$ has length $n$.
Every node of $Q_A$ ends up in $\top$ after following a prefix of $w^{(i)}$. Again, if it ended up in another node $\hat{q}$, the algorithm would have
performed another iteration and enlarging $R^{(i)}$; if there were no node that $q$ ended up in following a $w \in R$, a prefix of every $w \in R$ must have led it to $\top$ before.
We can conclude that every run $r$ with $\bar{r}|_G$ is a prefix of a word in $(AC)^* R (AC)^\omega$ is terminating, and thus $(AC)^* R (AC)^\omega$ is a terminating pattern.
\qed
\end{proof}





==> nondeterminism.tex <==
%%%%%%%%%%%%%%%


\section{Patterns for Nondeterministic Programs}
\label{sec:nondetpatterns}


\subsection{Action Patterns}
\begin{figure}[tbp]
\centering
 \tikzset{
   dim/.style={
           rounded corners,
           minimum height=2em,
           inner sep=2pt,
           text centered,
           },
    state/.style={
           rectangle,
           rounded corners,
           draw=black, very thick,
           minimum height=2em,
           inner sep=2pt,
           text centered,
           },
   act/.style={
           circle,
           draw=black, very thick,
           minimum height=2em,
           inner sep=2pt,
           text centered,
           },
  fail/.style={circle, double, draw=black, inner sep=2pt, minimum height=2em, very thick},
  nothing/.style={
           rectangle,
           rounded corners,
           minimum height=2em,
           inner sep=0pt,
           text centered,
           }
  }
\scalebox{0.6}{
\centering
\begin{tikzpicture}[->,>=stealth',scale=1,font=\Large]

 \node[dim, anchor=center] (S1)
 {$ $};

 \node[act] (L0) [right =of S1]
 {$\bot$};

 \node[act] (L1) [right =3.5cm of L0]
 {$l_1$};

 \node[act] (L2) [right =3.5cm of L1]
 {$l_2$};

 \node[act] (TOP) [right =3cm of L2]
 {$\top$};

 % draw the paths and and print some Text below/above the graph
 \path[very thick]
       (S1) edge[above] node [above] {$ $} (L0)
       (L0) edge[above] node [below] {$x := \nondet()$} (L1)
       (L1) edge[above] node [below] {$y := \coin(p)$} (L2)
       (L2) edge node [below] {$x \not= y?$} (TOP)
        (L2) edge[bend right=25] node [above] {$x = y?$} (L0)
       (TOP) edge[loop below] node [right] {} (TOP);
\end{tikzpicture}
}
\caption{A.s.-terminating program without terminating coin pattern.}\label{fig:coinPatternCounterExample}
\end{figure}
%
For general a.s.-terminating probabilistic programs, there might not exist a terminating pattern, even if
the program is finite.
As an example, consider the a.s.-terminating program $P$ given in Fig.~\ref{fig:coinPatternCounterExample}.

Its only starting configuration $\sigma_0$ is defined by
\stefan{starting configuration is irrelevant, oder?}
$\sigma_0(x) = \sigma_0(y) = 0$.
%
Assume for the sake of contradiction that there exists a terminating pattern $\Phi = C^*w_1C^*w_2C^*\ldots$ for $P$.
Let $c_1 c_2 c_3 \ldots \in \Phi$.
%Define a map $\widetilde{\cdot}: C \rightarrow Lab_A$ by setting $\widetilde{i} = a_i$, for $i \in \{0,1\}$.
The run
\begin{equation*}
 \tup{\bot, \sigma_0}
 \xrightarrow {a_{c_1}}
 \tup{l_1, \sigma_1}
 \xrightarrow  {c_1}
 \tup{l_2, \sigma'_1}
 \xrightarrow \tau
 \tup{\bot, \sigma'_1}
 \xrightarrow  {a_{c_2}}
 \tup{l_1, \sigma_2}
 \xrightarrow  {c_2}
 \tup{l_2, \sigma'_2}
 \xrightarrow \tau
 \tup{\bot, \sigma'_2}
 \xrightarrow  {a_{c_3}}
 \ldots
\end{equation*}
in $\mathcal{M}_P$ is $\Phi$-conforming but nonterminating. %, but is contained in $\Runs(\Phi, C)$.
%Intuitively, regardless how the coin toss outcomes are chosen,
%the nondeterministic choices can be adapted according to
%the succeding coin toss outcome.

We therefore propose another pattern class that also takes nondeterministic decisions into account.
We fix an arbitrary probabilistic program~$P = (\mathcal{L}, I, \mathord{\hookrightarrow}, \lab, \bot, \top)$,
and its associated MDP $\mathcal{M}_P =  (Q_A, Q_P, \text{Init}, \mathord{\rightarrow}, \text{Lab}_A, \text{Lab}_P)$.
We assume that $P$ is in a special \emph{normal form}: Every nondeterministic location has a probabilistic location as its successor, every
probabilistic location has a nondeterministic location as its successor. It is easy to transform a program in normal form by adding
redundant probabilistic and nondeterministic locations such that the transformed program terminates if{}f the original one does.
For example, the program in Fig.~\ref{fig:coinPatternCounterExample} is in normal form.
%Note that for every run $r \in \mathcal{M}_P$, it holds that $r|_G \in (A C)^\infty$ if $P$ is in normal form.
If $P$ is in normal form, then every run $r \in \mathcal{M}_P$ satisfies $r|_G \in (A C)^\infty$.

We write $A := \{a_0, a_1\}$ and $G := \{a_0, a_1\} \cup C$.
A set $W \subseteq (A C)^*$ is called a \emph{response} of length~$n \geq 0$ if
(i) every $w \in W$  has length $2n$,
(ii) for $w_1, w_2 \in W$ with $w_1 \not= w_2$, $w_1|_A \not= w_2|_A$ holds, and (iii) $W$ contains exactly $2^n$ elements.
We denote by $\Resp(n)$ the set of responses of length~$n$, and set $\Resp := \bigcup_{n \in \mathbb{N}}{\Resp(n)}$.
Intuitively, a response $R$ of length~$n$ contains for every sequence of nondeterministic actions of length $n$ a sequence of
coin toss outcomes of length $n$ (interleaved in one word of $R$). For example,
$\{a_0c_1, a_1c_0\}$ is a response of length one, $\{a_0c_0a_0c_1, a_0c_0a_1c_1, a_1c_0a_0c_1, a_1c_0a_1c_1\}$ is a response
of length two.
%
% \begin{example}
% \label{ex:responseSeq}
% $\emptyset$ is the only response of length 0,
% $W = \{a_0c_1, a_1c_0\}$ is a response of length one. An example for a response of length two is
% $W' = \{a_0c_0a_0c_1, a_0c_0a_1c_1, a_1c_0a_0c_1, a_1c_0a_1c_1\}$.
% \end{example}


A \emph{response pattern} is a subset of $(A C)^\omega$ of the form $(A C)^* R_1 (A C)^* R_2 (A C)^* \ldots$, where $R_1, R_2, \ldots$ are responses.
We say $R_1, R_2, \ldots$ induces the response pattern.

%A response pattern of the form $(A C)^* R (A C)^* R (A C)^* \ldots$ for $R$ a response is said to be \emph{simple}.
As in the deterministic case,
fixing an enumeration $R_1, R_2, \ldots$ of all responses, we call the pattern $(A C)^* R_1 (A C)^*R_2(A C)^*$ a \emph{universal response pattern}.
For a response pattern~$\Phi$, a run $r \in \Runs(\mathcal{M}_P)$ is $\Phi$-conforming if there is $v \in \Phi$ such that $\bar{r}|_G$ is a prefix of $v$.
We call a response pattern $\Phi$ \emph{terminating} if all $\Phi$-conforming runs terminate.

Analogously to the deterministic case,
we show the following theorem:
\newcommand{\stmtthmresponsePattern}{
Let $P$ be a probabilistic program in normal form.
\begin{itemize}
\item[(1)]
 Let $\Phi$ be a response pattern.
 The set of $\Phi$-conforming runs has probability~$1$ for every strategy $S$ for $\mathcal{M}_P$.
 In particular, if $P$ has a terminating pattern, then $P$ is a.s.-terminating.
\item[(2)]
 If $P$ is a.s.-terminating and weakly finite, then the universal pattern is terminating for~$P$.
\item[(3)]
 If $P$ is a.s.-terminating and finite with $n < \infty$ reachable nodes in~$\mathcal{M}_P$,
  then there exists a response $R$ of length in $\mathcal{O}(n^2)$ such that $(A C)^* R (A C)^\omega$ is terminating for~$P$.
\end{itemize}
}
\begin{theorem} \label{th:responsePattern}
 \stmtthmresponsePattern
\end{theorem}

The proof of Theorem~\ref{th:responsePattern} is similar to the one of Theorem~\ref{th:coinPattern} and can be found in the appendix.

% \begin{proof}[of Theorem~\ref{th:responsePattern}] \\
% Part~(1)~(Sketch): Let $\Phi = (A C)^*R_1(A C)^*R_2(A C)^* \ldots$ be a response pattern, and let $\Phi_1 = (A C)^* R_1 (A C)^\omega$ with $R_1$ of length $n$.
% %All runs containing only finitely many coin tosses are conforming to $\Phi_1$.
% We fix a strategy $S$ for $\mathcal{M}_P$.
% Let $p_{\min}$ be defined as in Theorem~\ref{th:coinPattern}.
% $R_1$ gives for every possible choice of action labels of length $n$ a corresponding coin sequence.
% Hence, regardless of the labels chosen by strategy $S$, for each action node $q$ and each run starting in $q$, the probability of visiting \emph{one} of the sequences $w \in R_1$ at the beginning of the run or only visiting finitely many
% nondeterministic (and probabilistic) nodes is greater or equal than $p_{\min}^{\abs{w_1}} > 0$. The set of runs $r$ that visit infinitely many nondeterministic nodes and do not contain an element of $R_1$ as substring of $r|_G$ is therefore again a null set.
% This result can be easily generalized to sets of the form $(A C)^* w_1 (A C)^* w_2 \ldots (A C)^* w_n (A C)^\omega$. $\Phi$ can then be formed as the countable intersection of these patterns.
%
% Part~(2): The proof is analogously to the one of Theorem~\ref{th:coinPattern}, part (2).
%
% Part~(3)~(Sketch): Since $P$ is a.s.-terminating, for every node $q \in Q_A$ and every sequence $x = x_1 x_2 \ldots x_n \in A^n$  there exists a coin toss sequence $w_q = c_1 c_2 \ldots c_n$ with
% the following property: a run that passes through $q$ and afterwards visits a label sequence of the form $\tau^* x_1 c_0 \tau^* x_1 c_1 \tau^* \ldots \tau^* x_n c_n$  (or a maximal possible prefix thereof)
% is terminating. Otherwise, there would exist a strategy such that, after visiting $q$, no run is able to reach $\top$.
% The set of words $x_1 c_1 \ldots x_n c_n$ for a fixed state $q$ form a response $R_q$ of length $n$. Again we construct a composed response $R$ out of these $R_q$'s of length maximal $n^2$
% such that for every state $q$ every run that passes through $q$ and then visits \emph{one of the words} in $R$ is terminating.
% \qed
% \end{proof}
% %




\begin{example}
 For the program in Fig.~\ref{fig:coinPatternCounterExample}, a terminating response pattern is $\Phi = (A C)^* \{a_0c_1, a_1c_0\} (A C)^\omega$.
  Every $\Phi$-conforming run has the form
\begin{equation*}
 \tup{\top, \sigma_0} \rightarrow \ldots \rightarrow q \xrightarrow {a_{i} } q' \xrightarrow {c_{1-i}} q'' \rightarrow \top  \rightarrow \ldots
 \qquad \text{for an $i \in \{0,1\}$.}
\end{equation*}
\end{example}



